Barren plateaus from learning scramblers with local cost functions

The existence of barren plateaus has recently revealed new training challenges in quantum machine learning (QML). Uncovering the mechanisms behind barren plateaus is essential in understanding the scope of problems that QML can efficiently tackle. Barren plateaus have recently been shown to exist when learning global properties of random unitaries, which is relevant when learning black hole dynamics. Establishing whether local cost functions can circumvent these barren plateaus is pertinent if we hope to apply QML to quantum many-body systems. We prove a no-go theorem showing that local cost functions encounter barren plateaus in learning random unitary properties.

==> GlobalCost.tex <==
\section{Global versus local cost functions}
In \cite{Holmes2021}, the global cost function used to learn a unitary $V$ is
\begin{equation}
	C_g=\bra{\psi}U^\dagger V H V^\dagger U\ket{\psi} ,
\end{equation}
where $H$ is a Hermitian operator, which may be local. The cost function is optimized such that $U=V$, i.e., $U$ learns $V$ globally. Although $H$ may be local, $V H V^\dagger$ is typically global if $V$ is a scrambler. One therefore expects $C_g$ to exhibit a barren plateau. One may try to construct a similar cost function which resembles a local function:
\begin{equation}
	C_g'=\bra{\psi}VU^\dagger  H UV^\dagger \ket{\psi}.
\end{equation}
The state is prepared by applying $V^\dagger$ to $\ket{\psi}$ followed by $U$. One can then measure the local observable $H$ in this state. For simplicity, assume $H=\ket{0}\bra{0}\otimes I_d^{\otimes n-1}$. At first glance, $C_g'$ appears to be a local cost function, since the observable $H$ is local. However, upon rewriting the cost function as
\begin{equation}
	C'_g=d^{n-1}\tr{
	U^\dagger  (\frac{1}{d^{n-1}}H) UV^\dagger \ket{\psi}\bra{\psi}V},
\end{equation}
one can view $U^\dagger (\frac{1}{d^{n-1}}H)U$ as the evolved input state and $V^\dagger \ket{\psi}\bra{\psi}V$ as the global observable. Hence, $C'_g$ still qualifies as a global cost function.




